Adopting AI: How Familiarity Breeds Both Trust and Contempt

Despite pronouncements about the inevitable diffusion of artificial intelligence and autonomous technologies, in practice it is human behavior, not technology in a vacuum, that dictates how technology seeps into -- and changes -- societies. In order to better understand how human preferences shape technological adoption and the spread of AI-enabled autonomous technologies, we look at representative adult samples of US public opinion in 2018 and 2020 on the use of four types of autonomous technologies: vehicles, surgery, weapons, and cyber defense. By focusing on these four diverse uses of AI-enabled autonomy that span transportation, medicine, and national security, we exploit the inherent variation between these AI-enabled autonomous use cases. We find that those with familiarity and expertise with AI and similar technologies were more likely to support all of the autonomous applications we tested (except weapons) than those with a limited understanding of the technology. Individuals that had already delegated the act of driving by using ride-share apps were also more positive about autonomous vehicles. However, familiarity cut both ways; individuals are also less likely to support AI-enabled technologies when applied directly to their life, especially if technology automates tasks they are already familiar with operating. Finally, opposition to AI-enabled military applications has slightly increased over time.

==> tables/SummaryStatistics2018.tex <==
Gender              &     1000.00&        0.58&        0.49&        0.00&        1.00\\
Age                 &     1000.00&       49.03&       17.75&       19.00&       96.00\\
White               &     1000.00&        0.74&        0.44&        0.00&        1.00\\
Level of Education  &     1000.00&        3.63&        1.54&        1.00&        6.00\\
Family Income       &      901.00&        6.28&        3.34&        1.00&       16.00\\
Partisanship: 1 = Dem, 7 = GOP&      960.00&        3.72&        2.24&        1.00&        7.00\\
Top 10 Auto Manufacturing State&     1000.00&        0.18&        0.39&        0.00&        1.00\\
Top 10 HC Employment State&     1000.00&        0.08&        0.27&        0.00&        1.00\\
Prior AI Knowledge  &     1000.00&        0.47&        0.71&        0.00&        2.00\\
Current or Prior Military Service&     1000.00&        0.11&        0.31&        0.00&        1.00\\
Urban Area          &      992.00&        2.24&        1.06&        1.00&        4.00\\

==> tables/SummaryStatistics2020.tex <==
Gender              &     1000.00&        0.56&        0.50&        0.00&        1.00\\
Age                 &     1000.00&       49.29&       17.64&       19.00&       89.00\\
White               &     1000.00&        0.72&        0.45&        0.00&        1.00\\
Level of Education  &     1000.00&        3.61&        1.49&        1.00&        6.00\\
Family Income       &      913.00&        6.32&        3.45&        1.00&       16.00\\
Partisanship: 1 = Dem, 7 = GOP&      951.00&        3.48&        2.18&        1.00&        7.00\\
Top 10 Auto Manufacturing State&     1000.00&        0.17&        0.37&        0.00&        1.00\\
Top 10 HC Employment State&     1000.00&        0.08&        0.27&        0.00&        1.00\\
Prior AI Knowledge  &     1000.00&        1.26&        1.13&        0.00&        5.00\\
Personal AI Use: 1 = home or work 2 = home/work&     1000.00&        0.33&        0.61&        0.00&        2.00\\
Pre-COVID Ridesharing Use&      933.00&        1.60&        0.90&        1.00&        5.00\\
Drivers License     &      997.00&        0.88&        0.33&        0.00&        1.00\\
Current or Prior Military Service&     1000.00&        0.11&        0.31&        0.00&        1.00\\
Urban Area          &      995.00&        2.20&        1.05&        1.00&        4.00\\
COVID-19 Death Family/Friends&     1000.00&        0.16&        0.37&        0.00&        1.00\\
